Iterative Classification of Graph-Set-Based Designs (IC-GSBD) for the Down-Selection of Aircraft Thermal Management Systems

In this paper, we present Iterative Classification of Graph-Set-Based Design (IC-GSBD), a framework utilizing graph-based techniques with geometric deep learning (GDL) integrated within a set-based design (SBD) approach for the classification and down-selection complex engineering systems represented by graphs. We demonstrate this approach on aircraft thermal management systems (TMSs) utilizing previous datasets created using an enumeration or brute-force graph generation procedure to represent novel aircraft TMSs as graphs. However, as with many enumerative approaches, combinatorial explosion limits its efficacy in many real-world problems, particularly when simulations and optimization must be performed on the many (automatically-generated) physics models. Therefore, the approach uses the directed graphs representing aircraft TMSs and GDL to predict on a subset of the graph-based dataset through graph classification. This paper's findings demonstrate that incorporating additional graph-based features using principle component analysis (PCA) enhances GDL model performance, achieving an accuracy of 98% for determining a graph's compilability and simulatability while using only 5% of the data for training. By applying iterative classification methods, we also successfully segmented the total set of graphs into more specific groups with an average inclusion of 75.5 of the top 100 highest-performing graphs, achieved by training on 40% of the data.

==> input/background/sbd_comparison_fig.tex <==
% \begin{figure}
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \begin{tikzpicture}[node distance=1.8cm, scale=0.65, every node/.style={transform shape}]
%             \node (start) [process] {Define Requirements and Constraints};
%             \node (generate) [process, below of=start] {Generate Initial Design Alternatives};
%             \node (analyze) [process, below of=generate] {Analyze and Evaluate Design Alternatives};
%             \node (narrow) [process, below of=analyze] {Narrow Down Design Alternatives};
%             \node (decision) [decision, below of=narrow, yshift=-0.5cm] {Does the design meet stakeholder needs?};
%             \node (refine) [process, left of=decision, xshift=-3.5cm] {Iteratively Refine Alternatives};
%             \node (final) [process, below of=decision, yshift=-0.8cm] {Finalize Design and Develop Detailed Specifications};
%             % \node (improve) [process, below of=final] {Continuous Improvement and Feedback};
        
%             \draw [arrow] (start) -- (generate);
%             \draw [arrow] (generate) -- (analyze);
%             \draw [arrow] (analyze) -- (narrow);
%             \draw [arrow] (narrow) -- (decision);
%             \draw [arrow] (decision) -- node[anchor=east] {yes} (final);
%             \draw [arrow] (decision) -- node[anchor=south] {no} (refine);
%             \draw [arrow] (refine) |- (generate);
%             % \draw [arrow] (final) -- (improve);
%             % \draw [arrow] (improve) -| ([xshift=2cm]generate.east) -- (generate);
%         \end{tikzpicture}
%         \label{fig:sbdflow}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \begin{tikzpicture}[node distance=1.8cm, scale=0.65, every node/.style={transform shape}]
%             \node (start) [process] {Define Requirements and Constraints};
%             \node (generate) [dygide, below of=start] {Generate Graph-Based Architectures Set};
%             \node (analyze2) [dygide, below of=generate] {Analyze and Evaluate a Fraction of the Dataset};            
%             \node (train) [dygide, below of=analyze2] {Train GDL Model};
%             % \node (analyze) [dygide, below of=train] {Analyze and Evaluate Design Alternatives}; 
%             \node (narrow) [dygide, below of=train] {Narrow Down Design Alternatives};
                       
%             \node (decision) [decision, below of=narrow, yshift=-0.5cm] {Does the design meet stakeholder needs?};
%             \node (refine) [process, left of=decision, xshift=-3.5cm] {Iteratively Refine Alternatives};
%             \node (final) [process, below of=decision, yshift=-0.8cm] {Finalize Design and Develop Detailed Specifications};
%             % \node (improve) [process, below of=final] {Continuous Improvement and Feedback};
            
        
%             \draw [arrow] (start) -- (generate);
%             \draw [arrow] (generate) -- (analyze2);
%             \draw [arrow] (analyze2) -- (train);
%             \draw [arrow] (train) -- (narrow);
%             \draw [arrow] (narrow) -- (decision);
%             \draw [arrow] (decision) -- node[anchor=east] {yes} (final);
%             \draw [arrow] (decision) -- node[anchor=south] {no} (refine);
%             \draw [arrow] (refine) |- (generate);
%             % \draw [arrow] (final) -- (improve);
%             % \draw [arrow] (improve) -| ([xshift=3.5cm]generate.east) -- (generate);
%             \draw [arrow] (narrow) -| ([xshift=1.5cm]train.east) -- (train);

%             \begin{scope}[on background layer]
%                 \node (box) [draw=black, dashed, fit=(train) (narrow), inner sep=8pt, label=above right:Machine Learning Process] {};
%             \end{scope}
%         \end{tikzpicture}
%         \label{fig:dygideflow}  
%     \end{subfigure}
%     \caption{Comparison of traditional SBD workflow and DyGIDE enhanced SBD workflow.}

% \end{figure}

\begin{figure}[t]
    \centering
    \begin{tikzpicture}[node distance=1.8cm, scale=0.65, every node/.style={transform shape}]
        \node (start) [process] {Define Requirements and Constraints};
        \node (generate) [process, below of=start] {Generate Initial Design Alternatives};
        \node (analyze) [process, below of=generate] {Analyze and Evaluate Design Alternatives};
        \node (narrow) [process, below of=analyze] {Narrow Down Design Alternatives};
        \node (decision) [decision, below of=narrow, yshift=-0.5cm] {Does the design meet stakeholder needs?};
        \node (refine) [process, left of=decision, xshift=-3.5cm] {Iteratively Refine Alternatives};
        \node (final) [process, below of=decision, yshift=-0.8cm] {Finalize Design and Develop Detailed Specifications};
        % \node (improve) [process, below of=final] {Continuous Improvement and Feedback};
    
        \draw [arrow] (start) -- (generate);
        \draw [arrow] (generate) -- (analyze);
        \draw [arrow] (analyze) -- (narrow);
        \draw [arrow] (narrow) -- (decision);
        \draw [arrow] (decision) -- node[anchor=east] {yes} (final);
        \draw [arrow] (decision) -- node[anchor=south] {no} (refine);
        \draw [arrow] (refine) |- (generate);
        % \draw [arrow] (final) -- (improve);
        % \draw [arrow] (improve) -| ([xshift=2cm]generate.east) -- (generate);
    \end{tikzpicture}
    \label{fig:sbdflow}
    \caption{The workflow for Set-Based Design.}
\end{figure}

==> input/case_study/intro.tex <==
A TMS controls the temperatures of two hypothetical loads: a flight control heat load and a radar heat load. 
The designated target temperatures are 343K for the flight control and 300K for the radar. 
A multi-objective utility function ranks and selects the most suitable architectural designs. 
This function considers various goals, including keeping thermal loads within specified temperature ranges. The utility function is defined as follows:

\begin{eqnarray}
    \text{minimize: } J &=& w_1j_1 + w_2j_2 + w_3j_3 + w_4j_4 + w_5j_5\\
     &=& w_1 (\bar{T}_{HLF} - 343K) + w_2(\bar{T}_{HLR} - 300K) + w_3 C_{total} + w_4\dot{m}_{BSI} + w_5\dot{m}_{RSI}
\end{eqnarray}

In this function, \(\bar{T}_{HLF}\) represents the average temperature of the flight control heat load, \(\bar{T}_{HLR}\) is for the radar heat load, \(C_{total}\) denotes the total heat capacity of the heat exchangers, and \(\dot{m}_{BSI}\) and \(\dot{m}_{RSI}\) are the mass flow rates of the bleed air and ram air, respectively. Nominal weights have been established to provide a singular value for ranking different architectural solutions.

Employing the techniques outlined in \sref{enum} and \rref{herber2020}, a total of 32,612 potential Thermal Management System (TMS) architectures were produced. These architectures were assessed using 200 parameter sets, randomly generated based on adjustable system parameters. It's noteworthy that this evaluation process spanned over nine days. Of the generated graphs, 5,585 were successfully compiled, and 2,098 could be simulated among these.
